Do the Machine Learning Models on a Crowd Sourced Platform Exhibit Bias? An Empirical Study on Model Fairness

Machine learning models are increasingly being used in important decision-making software such as approving bank loans, recommending criminal sentencing, hiring employees, and so on. It is important to ensure the fairness of these models so that no discrimination is made based on protected attribute (e.g., race, sex, age) while decision making. Algorithms have been developed to measure unfairness and mitigate them to a certain extent. In this paper, we have focused on the empirical evaluation of fairness and mitigations on real-world machine learning models. We have created a benchmark of 40 top-rated models from Kaggle used for 5 different tasks, and then using a comprehensive set of fairness metrics, evaluated their fairness. Then, we have applied 7 mitigation techniques on these models and analyzed the fairness, mitigation results, and impacts on performance. We have found that some model optimization techniques result in inducing unfairness in the models. On the other hand, although there are some fairness control mechanisms in machine learning libraries, they are not documented. The mitigation algorithm also exhibit common patterns such as mitigation in the post-processing is often costly (in terms of performance) and mitigation in the pre-processing stage is preferred in most cases. We have also presented different trade-off choices of fairness mitigation decisions. Our study suggests future research directions to reduce the gap between theoretical fairness aware algorithms and the software engineering methods to leverage them in practice.

==> discussion.tex <==
\section{Discussion}
\label{sec:discussion}
The following outline for a paper that introduces a technical idea.


==> main-table-backup.tex <==
\begin{table*}[!h]
	\footnotesize
	\centering
	\caption{Model unfairness measures and mitigations}
	\label{tab:main}%
	\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|}
		\hline
		\rowcolor[HTML]{EFEFEF} 
		\multicolumn{1}{|c|}{\cellcolor[HTML]{EFEFEF}}                                & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}}                                 & \multicolumn{9}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{Before Mitigation}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                & \multicolumn{9}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{After Mitigation}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                 \\ \hhline{|~|~|*{18}{-}} 
		\rowcolor[HTML]{EFEFEF} 
		\multicolumn{1}{|c|}{\multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}\textbf{Data}}} & \multicolumn{1}{c|}{\multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}\textbf{Model}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{Acc}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{F1}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{DI}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{SPD}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{EOD}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{AOD}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{ERD}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{CNT}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{TI}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{Acc}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{F1}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{DI}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{SPD}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{EOD}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{AOD}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{ERD}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{CNT}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{TI}}\\ \hline
		& GC1-RFT                                               & 0.687                                                     & 0.814                                                    & 0.002                                                    & 0.002                                                     & 0                                                         & 0.004                                                     & 0.052                                                     & -0.002                                                    & 0.058                                                    & \cellcolor{cellblue}0.683                             & \cellcolor{cellblue}0.811                            & \cellcolor{cellblue}0.002                            & \cellcolor{cellblue}0.002                             & \cellcolor{cellblue}0                                 & \cellcolor{cellblue}0.004                             & \cellcolor{cellblue}-0.032                            & \cellcolor{cellblue}-0.002                            & \cellcolor{cellblue}0.058                            \\ \hhline{|~|*{19}{-}}  
		& GC2-XGB                                               & 0.743                                                     & 0.828                                                    & -0.076                                                   & -0.058                                                    & -0.039                                                    & -0.036                                                    & 0.047                                                     & -0.282                                                    & 0.142                                                    & \cellcolor{cellgreen}0.709                             & \cellcolor{cellgreen}0.829                            & \cellcolor{cellgreen}0                                & \cellcolor{cellgreen}0                                 & \cellcolor{cellgreen}0                                 & \cellcolor{cellgreen}0                                 & \cellcolor{cellgreen}0.067                             & \cellcolor{cellgreen}0                                 & \cellcolor{cellgreen}0.057                            \\ \hhline{|~|*{19}{-}}  
		& GC3-XGB                                               & 0.742                                                     & 0.827                                                    & -0.105                                                   & -0.079                                                    & -0.043                                                    & -0.065                                                    & 0.036                                                     & -0.173                                                    & 0.149                                                    & \cellcolor{cellgreen}0.729                             & \cellcolor{cellgreen}0.831                            & \cellcolor{cellgreen}-0.045                           & \cellcolor{cellgreen}-0.04                             & \cellcolor{cellgreen}-0.006                            & \cellcolor{cellgreen}-0.043                            & \cellcolor{cellgreen}0.037                             & \cellcolor{cellgreen}-0.095                            & \cellcolor{cellgreen}0.1                              \\ \hhline{|~|*{19}{-}}  
		& GC4-SVM                                               & 0.753                                                     & 0.832                                                    & -0.138                                                   & -0.104                                                    & -0.081                                                    & -0.068                                                    & 0.07                                                      & -0.338                                                    & 0.153                                                    & \cellcolor{cellgreen}0.716                             & \cellcolor{cellgreen}0.834                            & \cellcolor{cellgreen}0                                & \cellcolor{cellgreen}0                                 & \cellcolor{cellgreen}0                                 & \cellcolor{cellgreen}0                                 & \cellcolor{cellgreen}0.09                              & \cellcolor{cellgreen}0                                 & \cellcolor{cellgreen}0.057                            \\ \hhline{|~|*{19}{-}}  
		& GC5-EVC                                               & 0.743                                                     & 0.826                                                    & -0.148                                                   & -0.116                                                    & -0.075                                                    & -0.089                                                    & 0.067                                                     & -0.286                                                    & 0.127                                                    & \cellcolor{cellgreen}0.687                             & \cellcolor{cellgreen}0.814                            & \cellcolor{cellgreen}0                                & \cellcolor{cellgreen}0                                 & \cellcolor{cellgreen}0                                 & \cellcolor{cellgreen}0                                 & \cellcolor{cellgreen}0.112                             & \cellcolor{cellgreen}0                                 & \cellcolor{cellgreen}0.058                            \\ \hhline{|~|*{19}{-}}  
		& GC6-RFT                                               & 0.761                                                     & 0.845                                                    & -0.103                                                   & -0.083                                                    & -0.023                                                    & -0.085                                                    & 0.005                                                     & -0.183                                                    & 0.121                                                    & \cellcolor{cellblue}0.759                             & \cellcolor{cellblue}0.844                            & \cellcolor{cellblue}-0.071                           & \cellcolor{cellblue}-0.058                            & \cellcolor{cellblue}-0.023                            & \cellcolor{cellblue}-0.085                            & \cellcolor{cellblue}-0.027                            & \cellcolor{cellblue}-0.183                            & \cellcolor{cellblue}0.121                            \\ \hhline{|~|*{19}{-}}  
		& GC7-XGB                                               & 0.751                                                     & 0.831                                                    & -0.073                                                   & -0.056                                                    & 0.009                                                     & -0.072                                                    & -0.033                                                    & -0.293                                                    & 0.144                                                    & \cellcolor{cellgreen}0.709                             & \cellcolor{cellgreen}0.829                            & \cellcolor{cellgreen}0                                & \cellcolor{cellgreen}0                                 & \cellcolor{cellgreen}0                                 & \cellcolor{cellgreen}0                                 & \cellcolor{cellgreen}0.047                             & \cellcolor{cellgreen}0                                 & \cellcolor{cellgreen}0.057                            \\ \hhline{|~|*{19}{-}}  
		\multirow{-8}{*}{\rotatebox{90}{\shortstack{German Credit* \\ (Sex)}}}                                  & GC8-KNN                                               & 0.698                                                     & 0.815                                                    & 0.003                                                    & 0.002                                                     & 0                                                         & 0.011                                                     & 0.081                                                     & -0.041                                                    & 0.09                                                     & \cellcolor{cellblue}0.702                             & \cellcolor{cellblue}0.825                            & \cellcolor{cellblue}0                                & \cellcolor{cellblue}0                                 & \cellcolor{cellblue}0                                 & \cellcolor{cellblue}0                                 & \cellcolor{cellblue}0.086                             & \cellcolor{cellblue}0                                 & \cellcolor{cellblue}0.057                            \\ \hline
		& AC1-LRG                                               & 0.845                                                     & 0.657                                                    & -0.654                                                   & -0.104                                                    & -0.1                                                      & -0.069                                                    & -0.05                                                     & -0.045                                                    & 0.127                                                    & \cellcolor{cellorange}0.261                             & \cellcolor{cellorange}0.399                            & \cellcolor{cellorange}0.023                            & \cellcolor{cellorange}0.023                             & \cellcolor{cellorange}0.017                             & \cellcolor{cellorange}0.021                             & \cellcolor{cellorange}0.12                              & \cellcolor{cellorange}-0.019                            & \cellcolor{cellorange}0.04                             \\ \hhline{|~|*{19}{-}}  
		& AC2-RFT                                               & 0.846                                                     & 0.657                                                    & -0.582                                                   & -0.098                                                    & -0.047                                                    & -0.046                                                    & -0.06                                                     & -0.236                                                    & 0.119                                                    & \cellcolor{cellgreen}0.787                             & \cellcolor{cellgreen}0.249                            & \cellcolor{cellgreen}-0.354                           & \cellcolor{cellgreen}-0.014                            & \cellcolor{cellgreen}0.007                             & \cellcolor{cellgreen}0.003                             & \cellcolor{cellgreen}-0.086                            & \cellcolor{cellgreen}-0.005                            & \cellcolor{cellgreen}0.232                            \\ \hhline{|~|*{19}{-}}  
		& AC3-GBC                                               & 0.858                                                     & 0.677                                                    & -0.496                                                   & -0.079                                                    & -0.041                                                    & -0.031                                                    & -0.045                                                    & -0.01                                                     & 0.12                                                     & \cellcolor{cellblue}0.858                             & \cellcolor{cellblue}0.675                            & \cellcolor{cellblue}-0.131                           & \cellcolor{cellblue}-0.024                            & \cellcolor{cellblue}-0.041                            & \cellcolor{cellblue}-0.031                            & \cellcolor{cellblue}-0.004                            & \cellcolor{cellblue}-0.01                             & \cellcolor{cellblue}0.12                             \\ \hhline{|~|*{19}{-}}  
		& AC4-CBC                                               & 0.869                                                     & 0.712                                                    & -0.616                                                   & -0.102                                                    & -0.077                                                    & -0.056                                                    & -0.044                                                    & -0.069                                                    & 0.107                                                    & \cellcolor{cellorange}0.805                             & \cellcolor{cellorange}0.683                            & \cellcolor{cellorange}-0.127                           & \cellcolor{cellorange}-0.044                            & \cellcolor{cellorange}0.08                              & \cellcolor{cellorange}0.044                             & \cellcolor{cellorange}-0.001                            & \cellcolor{cellorange}-0.102                            & \cellcolor{cellorange}0.082                            \\ \hhline{|~|*{19}{-}}  
		& AC5-XGB                                               & 0.867                                                     & 0.708                                                    & -0.588                                                   & -0.097                                                    & -0.073                                                    & -0.051                                                    & -0.043                                                    & -0.224                                                    & 0.111                                                    & \cellcolor{cellblue}0.865                             & \cellcolor{cellblue}0.705                            & \cellcolor{cellblue}-0.203                           & \cellcolor{cellblue}-0.039                            & \cellcolor{cellblue}-0.073                            & \cellcolor{cellblue}-0.051                            & \cellcolor{cellblue}-0.002                            & \cellcolor{cellblue}-0.224                            & \cellcolor{cellblue}0.111                            \\ \hhline{|~|*{19}{-}}  
		& AC6-XGB                                               & 0.871                                                     & 0.717                                                    & -0.57                                                    & -0.096                                                    & -0.044                                                    & -0.036                                                    & -0.047                                                    & -0.062                                                    & 0.106                                                    & \cellcolor{cellorange}0.808                             & \cellcolor{cellorange}0.691                            & \cellcolor{cellorange}-0.132                           & \cellcolor{cellorange}-0.046                            & \cellcolor{cellorange}0.072                             & \cellcolor{cellorange}0.044                             & \cellcolor{cellorange}0.009                             & \cellcolor{cellorange}-0.094                            & \cellcolor{cellorange}0.078                            \\ \hhline{|~|*{19}{-}}  
		& AC7-RFT                                               & 0.852                                                     & 0.678                                                    & -0.615                                                   & -0.104                                                    & -0.078                                                    & -0.059                                                    & -0.051                                                    & -0.235                                                    & 0.117                                                    & \cellcolor{cellgreen}0.638                             & \cellcolor{cellgreen}0.329                            & \cellcolor{cellgreen}-0.289                           & \cellcolor{cellgreen}-0.024                            & \cellcolor{cellgreen}-0.005                            & \cellcolor{cellgreen}-0.009                            & \cellcolor{cellgreen}-0.039                            & \cellcolor{cellgreen}-0.009                            & \cellcolor{cellgreen}0.187                            \\ \hhline{|~|*{19}{-}}  
		\multirow{-8}{*}{\rotatebox{90}{\shortstack{Adult Census* \\ (Race)}}}                                  & AC8-DCT                                               & 0.853                                                     & 0.675                                                    & -0.519                                                   & -0.086                                                    & -0.04                                                     & -0.035                                                    & -0.05                                                     & -0.068                                                    & 0.121                                                    & \cellcolor{cellblue}0.852                             & \cellcolor{cellblue}0.673                            & \cellcolor{cellblue}-0.153                           & \cellcolor{cellblue}-0.029                            & \cellcolor{cellblue}-0.04                             & \cellcolor{cellblue}-0.035                            & \cellcolor{cellblue}-0.01                             & \cellcolor{cellblue}-0.068                            & \cellcolor{cellblue}0.121                            \\ \hline
		& BM1-XGB                                               & 0.906                                                     & 0.582                                                    & 0.627                                                    & 0.087                                                     & 0.074                                                     & 0.053                                                     & 0.051                                                     & -0.078                                                    & 0.074                                                    & \cellcolor{cellblue}0.905                             & \cellcolor{cellblue}0.581                            & \cellcolor{cellblue}0.274                            & \cellcolor{cellblue}0.032                             & \cellcolor{cellblue}0.074                             & \cellcolor{cellblue}0.053                             & \cellcolor{cellblue}0.017                             & \cellcolor{cellblue}-0.078                            & \cellcolor{cellblue}0.074                            \\ \hhline{|~|*{19}{-}}  
		& BM2-LGB                                               & 0.908                                                     & 0.606                                                    & 0.593                                                    & 0.083                                                     & 0.004                                                     & 0.022                                                     & 0.069                                                     & -0.034                                                    & 0.072                                                    & \cellcolor{cellorange}0.772                             & \cellcolor{cellorange}0.498                            & \cellcolor{cellorange}0.076                            & \cellcolor{cellorange}0.026                             & \cellcolor{cellorange}-0.037                            & \cellcolor{cellorange}-0.037                            & \cellcolor{cellorange}-0.031                            & \cellcolor{cellorange}-0.04                             & \cellcolor{cellorange}0.066                            \\ \hhline{|~|*{19}{-}}  
		& BM3-GBC                                               & 0.908                                                     & 0.604                                                    & 0.688                                                    & 0.1                                                       & 0.083                                                     & 0.056                                                     & 0.051                                                     & -0.032                                                    & 0.072                                                    & \cellcolor[HTML]{FFCCC9}0.852                             & \cellcolor[HTML]{FFCCC9}0.529                            & \cellcolor[HTML]{FFCCC9}0.066                            & \cellcolor[HTML]{FFCCC9}0.013                             & \cellcolor[HTML]{FFCCC9}-0.059                            & \cellcolor[HTML]{FFCCC9}-0.052                            & \cellcolor[HTML]{FFCCC9}0.006                             & \cellcolor[HTML]{FFCCC9}-0.089                            & \cellcolor[HTML]{FFCCC9}0.078                            \\ \hhline{|~|*{19}{-}}  
		& BM4-XGB                                               & 0.887                                                     & 0.33                                                     & 0.81                                                     & 0.048                                                     & 0.067                                                     & 0.042                                                     & 0.074                                                     & -0.01                                                     & 0.111                                                    & \cellcolor{cellblue}0.887                             & \cellcolor{cellblue}0.328                            & \cellcolor{cellblue}0.442                            & \cellcolor{cellblue}0.022                             & \cellcolor{cellblue}0.067                             & \cellcolor{cellblue}0.042                             & \cellcolor{cellblue}0.001                             & \cellcolor{cellblue}-0.01                             & \cellcolor{cellblue}0.111                            \\ \hhline{|~|*{19}{-}}  
		& BM5-SVC                                               & 0.875                                                     & 0.175                                                    & 0.139                                                    & 0.003                                                     & -0.077                                                    & -0.031                                                    & 0.126                                                     & -0.032                                                    & 0.126                                                    & \cellcolor{cellpurple}0.873                             & \cellcolor{cellpurple}0.002                            & \cellcolor{cellpurple}0.139                            & \cellcolor{cellpurple}0                                 & \cellcolor{cellpurple}-0.001                            & \cellcolor{cellpurple}0                                 & \cellcolor{cellpurple}0.11                              & \cellcolor{cellpurple}0                                 & \cellcolor{cellpurple}0.136                            \\ \hhline{|~|*{19}{-}}  
		& BM6-GBC                                               & 0.908                                                     & 0.612                                                    & 0.698                                                    & 0.105                                                     & 0.03                                                      & 0.038                                                     & 0.076                                                     & -0.033                                                    & 0.071                                                    & \cellcolor{cellorange}0.795                             & \cellcolor{cellorange}0.521                            & \cellcolor{cellorange}0.11                             & \cellcolor{cellorange}0.034                             & \cellcolor{cellorange}-0.072                            & \cellcolor{cellorange}-0.053                            & \cellcolor{cellorange}-0.019                            & \cellcolor{cellorange}-0.039                            & \cellcolor{cellorange}0.065                            \\ \hhline{|~|*{19}{-}}  
		& BM7-XGB                                               & 0.91                                                      & 0.611                                                    & 0.713                                                    & 0.107                                                     & 0.051                                                     & 0.052                                                     & 0.072                                                     & -0.047                                                    & 0.07                                                     & \cellcolor{cellred}0.829                             & \cellcolor{cellred}0.485                            & \cellcolor{cellred}0.022                            & \cellcolor{cellred}0.004                             & \cellcolor{cellred}-0.037                            & \cellcolor{cellred}-0.044                            & \cellcolor{cellred}-0.007                            & \cellcolor{cellred}-0.122                            & \cellcolor{cellred}0.085                            \\ \hhline{|~|*{19}{-}}  
		\multirow{-8}{*}{\rotatebox{90}{\shortstack{Bank Marketing* \\ (Age)}}}                                  & BM8-RFC                                               & 0.899                                                     & 0.435                                                    & 0.834                                                    & 0.066                                                     & 0.091                                                     & 0.058                                                     & 0.064                                                     & -0.023                                                    & 0.097                                                    & \cellcolor{cellorange}0.795                             & \cellcolor{cellorange}0.462                            & \cellcolor{cellorange}0.289                            & \cellcolor{cellorange}0.042                             & \cellcolor{cellorange}-0.048                            & \cellcolor{cellorange}-0.027                            & \cellcolor{cellorange}0.005                             & \cellcolor{cellorange}-0.052                            & \cellcolor{cellorange}0.073                            \\ \hline
		& HC1-LGB                                               & 0.882                                                     & 0.246                                                    & 0.577                                                    & 0.047                                                     & 0.068                                                     & 0.053                                                     & 0.051                                                     & -0.11                                                     & 0.084                                                    & \cellcolor{cellgreen}0.436                             & \cellcolor{cellgreen}0.136                            & \cellcolor{cellgreen}-0.081                           & \cellcolor{cellgreen}0.005                             & \cellcolor{cellgreen}0.002                             & \cellcolor{cellgreen}0.003                             & \cellcolor{cellgreen}-0.001                            & \cellcolor{cellgreen}-0.009                            & \cellcolor{cellgreen}0.05                             \\ \hhline{|~|*{19}{-}}  
		& HC2-LGB                                               & 0.92                                                      & 0.093                                                    & -0.66                                                    & -0.005                                                    & -0.014                                                    & -0.009                                                    & -0.033                                                    & -0.012                                                    & 0.081                                                    & \cellcolor{cellred}0.919                             & \cellcolor{cellred}0.022                            & \cellcolor{cellred}0.089                            & \cellcolor{cellred}0                                 & \cellcolor{cellred}0.004                             & \cellcolor{cellred}0.002                             & \cellcolor{cellred}-0.033                            & \cellcolor{cellred}-0.002                            & \cellcolor{cellred}0.084                            \\ \hhline{|~|*{19}{-}}  
		& HC3-GNB                                               & 0.913                                                     & 0.01                                                     & 0.974                                                    & 0.999                                                     & 0.007                                                     & 0.005                                                     & 0.006                                                     & -2.449                                                    & 0                                                        & \cellcolor{cellorange}0.732                             & \cellcolor{cellorange}0.194                            & \cellcolor{cellorange}0.181                            & \cellcolor{cellorange}0.857                             & \cellcolor{cellorange}0.047                             & \cellcolor{cellorange}0.019                             & \cellcolor{cellorange}0.031                             & \cellcolor{cellorange}-2.285                            & \cellcolor{cellorange}0                                \\ \hhline{|~|*{19}{-}}  
		& HC4-XGB                                               & 0.919                                                     & 0.073                                                    & -0.846                                                   & 1                                                         & 0                                                         & 0                                                         & 0                                                         & -2.47                                                     & 0                                                        & \cellcolor{cellred}0.818                             & \cellcolor{cellred}0.065                            & \cellcolor{cellred}-0.25                            & \cellcolor{cellred}0.933                             & \cellcolor{cellred}-0.027                            & \cellcolor{cellred}-0.021                            & \cellcolor{cellred}-0.024                            & \cellcolor{cellred}-2.189                            & \cellcolor{cellred}0                                \\ \hhline{|~|*{19}{-}}  
		& HC5-CBC                                               & 0.87                                                      & 0.302                                                    & 0.744                                                    & 0.865                                                     & 0.085                                                     & 0.14                                                      & 0.106                                                     & -2.524                                                    & 0                                                        & \cellcolor{cellgreen}0.552                             & \cellcolor{cellgreen}0.075                            & \cellcolor{cellgreen}-0.134                           & \cellcolor{cellgreen}0.999                             & \cellcolor{cellgreen}-0.025                            & \cellcolor{cellgreen}-0.017                            & \cellcolor{cellgreen}-0.021                            & \cellcolor{cellgreen}-2.772                            & \cellcolor{cellgreen}0.001                            \\ \hhline{|~|*{19}{-}}  
		& HC6-CBC                                               & 0.918                                                     & 0                                                        & -0.694                                                   & 0                                                         & 0                                                         & 0                                                         & 0.029                                                     & 0                                                         & 0.085                                                    & \cellcolor{cellgreen}0.501                             & \cellcolor{cellgreen}0.076                            & \cellcolor{cellgreen}-0.694                           & \cellcolor{cellgreen}0                                 & \cellcolor{cellgreen}0                                 & \cellcolor{cellgreen}0                                 & \cellcolor{cellgreen}-0.001                            & \cellcolor{cellgreen}0                                 & \cellcolor{cellgreen}0.049                            \\ \hhline{|~|*{19}{-}}  
		& HC7-XGB                                               & 0.91                                                      & 0.211                                                    & 0.979                                                    & 0.953                                                     & 0.034                                                     & 0.089                                                     & 0.057                                                     & -2.526                                                    & 0                                                        & \cellcolor{cellpurple}0.909                             & \cellcolor{cellpurple}0.072                            & \cellcolor{cellpurple}0.414                            & \cellcolor{cellpurple}0.974                             & \cellcolor{cellpurple}0.007                             & \cellcolor{cellpurple}-0.034                            & \cellcolor{cellpurple}-0.012                            & \cellcolor{cellpurple}-2.449                            & \cellcolor{cellpurple}0                                \\ \hhline{|~|*{19}{-}}  
		\multirow{-8}{*}{\rotatebox{90}{\shortstack{Home Credit* \\ (Sex)}}}                                  & HC8-RFT                                               & 0.661                                                     & 0.239                                                    & 0.383                                                    & 0.719                                                     & 0.147                                                     & 0.129                                                     & 0.133                                                     & -2.449                                                    & 0.001                                                    & \cellcolor{cellred}0.645                             & \cellcolor{cellred}0.226                            & \cellcolor{cellred}0.337                            & \cellcolor{cellred}0.681                             & \cellcolor{cellred}0.133                             & \cellcolor{cellred}0.098                             & \cellcolor{cellred}0.112                             & \cellcolor{cellred}-2.426                            & \cellcolor{cellred}0.001                            \\ \hline
		& TM1-XGB                                               & 0.807                                                     & 0.72                                                     & -2.247                                                   & -0.705                                                    & -0.631                                                    & -0.559                                                    & -0.056                                                    & -0.341                                                    & 0.153                                                    & \cellcolor{cellorange}0.649                             & \cellcolor{cellorange}0.58                             & \cellcolor{cellorange}-0.082                           & \cellcolor{cellorange}-0.039                            & \cellcolor{cellorange}0.027                             & \cellcolor{cellorange}0.177                             & \cellcolor{cellorange}0.115                             & \cellcolor{cellorange}-0.272                            & \cellcolor{cellorange}0.189                            \\ \hhline{|~|*{19}{-}}  
		& TM2-RFT                                               & 0.816                                                     & 0.753                                                    & -2.013                                                   & -0.709                                                    & -0.635                                                    & -0.515                                                    & 0.022                                                     & -0.293                                                    & 0.142                                                    & \cellcolor{cellorange}0.644                             & \cellcolor{cellorange}0.566                            & \cellcolor{cellorange}-0.106                           & \cellcolor{cellorange}-0.045                            & \cellcolor{cellorange}0.059                             & \cellcolor{cellorange}0.166                             & \cellcolor{cellorange}0.023                             & \cellcolor{cellorange}-0.269                            & \cellcolor{cellorange}0.223                            \\ \hhline{|~|*{19}{-}}  
		& TM3-EBG                                               & 0.799                                                     & 0.725                                                    & -2.125                                                   & -0.674                                                    & -0.637                                                    & -0.514                                                    & -0.017                                                    & -0.333                                                    & 0.165                                                    & \cellcolor{cellorange}0.647                             & \cellcolor{cellorange}0.572                            & \cellcolor{cellorange}-0.108                           & \cellcolor{cellorange}-0.045                            & \cellcolor{cellorange}0.031                             & \cellcolor{cellorange}0.148                             & \cellcolor{cellorange}0.05                              & \cellcolor{cellorange}-0.317                            & \cellcolor{cellorange}0.223                            \\ \hhline{|~|*{19}{-}}  
		& TM4-LRG                                               & 0.8                                                       & 0.732                                                    & -2.439                                                   & -0.808                                                    & -0.729                                                    & -0.694                                                    & -0.051                                                    & -0.381                                                    & 0.144                                                    & \cellcolor{cellorange}0.658                             & \cellcolor{cellorange}0.577                            & \cellcolor{cellorange}-0.075                           & \cellcolor{cellorange}-0.034                            & \cellcolor{cellorange}0.072                             & \cellcolor{cellorange}0.16                              & \cellcolor{cellorange}0.038                             & \cellcolor{cellorange}-0.327                            & \cellcolor{cellorange}0.207                            \\ \hhline{|~|*{19}{-}}  
		& TM5-GBC                                               & 0.816                                                     & 0.74                                                     & -2.268                                                   & -0.708                                                    & -0.647                                                    & -0.542                                                    & -0.022                                                    & -0.357                                                    & 0.151                                                    & \cellcolor{cellorange}0.651                             & \cellcolor{cellorange}0.572                            & \cellcolor{cellorange}-0.087                           & \cellcolor{cellorange}-0.033                            & \cellcolor{cellorange}0.097                             & \cellcolor{cellorange}0.174                             & \cellcolor{cellorange}0.029                             & \cellcolor{cellorange}-0.332                            & \cellcolor{cellorange}0.205                            \\ \hhline{|~|*{19}{-}}  
		& TM6-XGB                                               & 0.804                                                     & 0.73                                                     & -1.948                                                   & -0.665                                                    & -0.583                                                    & -0.499                                                    & -0.042                                                    & -0.345                                                    & 0.146                                                    & \cellcolor{cellorange}0.625                             & \cellcolor{cellorange}0.568                            & \cellcolor{cellorange}-0.079                           & \cellcolor{cellorange}-0.038                            & \cellcolor{cellorange}0.075                             & \cellcolor{cellorange}0.157                             & \cellcolor{cellorange}0.092                             & \cellcolor{cellorange}-0.367                            & \cellcolor{cellorange}0.19                             \\ \hhline{|~|*{19}{-}}  
		& TM7-RFt                                               & 0.825                                                     & 0.747                                                    & -2.232                                                   & -0.639                                                    & -0.555                                                    & -0.411                                                    & -0.029                                                    & -0.285                                                    & 0.161                                                    & \cellcolor{cellorange}0.653                             & \cellcolor{cellorange}0.577                            & \cellcolor{cellorange}-0.099                           & \cellcolor{cellorange}-0.043                            & \cellcolor{cellorange}0.1                               & \cellcolor{cellorange}0.188                             & \cellcolor{cellorange}0.003                             & \cellcolor{cellorange}-0.261                            & \cellcolor{cellorange}0.219                            \\ \hhline{|~|*{19}{-}}  
		\multirow{-8}{*}{\rotatebox{90}{\shortstack{Titanic ML* \\ (Sex)}}}                                  & TM8-RFT                                               & 0.814                                                     & 0.732                                                    & -2.306                                                   & -0.716                                                    & -0.633                                                    & -0.563                                                    & -0.051                                                    & -0.321                                                    & 0.149                                                    & \cellcolor{cellorange}0.649                             & \cellcolor{cellorange}0.596                            & \cellcolor{cellorange}-0.082                           & \cellcolor{cellorange}-0.042                            & \cellcolor{cellorange}0.011                             & \cellcolor{cellorange}0.166                             & \cellcolor{cellorange}0.157                             & \cellcolor{cellorange}-0.327                            & \cellcolor{cellorange}0.172                            \\ \hline
	\end{tabular}
	\\
	*Experiment has been conducted for multiple protected attributes; Among multiple mitigation techniques applied to the models, the most successful algorithms: \\
	\colorbox{cellblue}{Reweighing} \colorbox{cellsteel}{Disparate Impact Remover} \colorbox{cellgreen}{Adversarial Debiasing} \colorbox{cellgold}{Prejudice Remover} \colorbox{cellpurple}{Equalized Odds} \colorbox{cellred}{Calibrated Equalized Odds} \colorbox{cellorange}{Reject Option Classification}\\
	RFT: Random Forest, XGB: XGBoost, SVC: Support Vector Classifier, EVC: Ensemble Voting Classifier, KNN: K-Nearest Neighbors, LRG: Logistic Regression, GBC: Gradient Boosting Classifier, CBC: Cat Boost Classifier, DCT: Decision Treee, LGB: Light Gradient Boost, GNB: Gaussian Naive Bayes, EBG: Ensemble Bagging
\end{table*}%
